OSDP: Optimal Sharded Data Parallel for Distributed Deep Learning

Large-scale deep learning models contribute to significant performance improvements on varieties of downstream tasks. Current data and model parallelism approaches utilize model replication and partition techniques to support the distributed training of ultra-large models. However, directly deploying these systems often leads to sub-optimal training efficiency due to the complex model architectures and the strict device memory constraints. In this paper, we propose Optimal Sharded Data Parallel (OSDP), an automated parallel training system that combines the advantages from both data and model parallelism. Given the model description and the device information, OSDP makes trade-offs between the memory consumption and the hardware utilization, thus automatically generates the distributed computation graph and maximizes the overall system throughput. In addition, OSDP introduces operator splitting to further alleviate peak memory footprints during training with negligible overheads, which enables the trainability of larger models as well as the higher throughput. Extensive experimental results of OSDP on multiple different kinds of large-scale models demonstrate that the proposed strategy outperforms the state-of-the-art in multiple regards. Our code is available at https://github.com/Youhe-Jiang/OptimalShardedDataParallel.

==> approach.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=1.0\linewidth]{figure/DPvsZDP.png}
\caption{Operator processing in DP and ZDP mode.}
\label{fig:DPvsZDP}
\end{figure}

\section{OSDP: Optimal Sharded Data Parallel}
% OSDP proposes an adaptive redundancy data parallel system that guarantees both memory and training efficiency as well as breaks the memory bottlenecks of existing data parallel implementations. 
In this section, we first introduce the overall system design of OSDP, then propose operator splitting.


% \begin{figure}
% \centering
% \includegraphics[width=1\textwidth]{figure/OSDPworkflow.png}
% \caption{Workflow of OSDP.}
% \label{fig:ASDPS}
% \end{figure}

% \begin{algorithm}[tb]
% \caption{Optimal Sharded Data Parallel (OSDP)}
% \label{alg:CPSA}
% \textbf{Input}: Model Description MD, Device Information DI; \\
% \textbf{Output}:
% \begin{algorithmic}[1] %[1] enables line numbers
% \STATE \textit{//Iteratively increase the training batch size.} 
% \FOR{traing\_batch\_size $\in$ max\_int}
% \STATE \textit{//Profile and generate cost.}
% \STATE time\_cost, memory\_cost = Profiler(MD, DI, training\_batch\_size);
% \STATE \textit{//Generate plan and estimated throughput.}
% \STATE plan, throughput = Search\_Engine(time\_cost, memory\_cost);
% \STATE cand\_throughput.append(throughput), cand\_plan.append(plan);
% \STATE //Stop while all plans exceed memory limit.
% \IF{plan == None}
% \STATE \textbf{return} 0
% \ENDIF
% \ENDFOR
% \STATE \textit{//Filter out the optimal execution plan.}
% \STATE optimal\_plan = cand\_plan[index(max(cand\_throughput))];
% \STATE \textbf{return} optimal\_plan
% \end{algorithmic}
% \end{algorithm}


\subsection{Optimal Sharded Data Parallel} \label{sec:OSDP}

% OSDP is proposed to make trade-offs between the memory consumption reduction and the hardware efficiency improvement, which maximizes the system throughput. It provides two modes for processing each operator: Data Parallel (DP) and Zero redundancy Data Parallel (ZDP), and an execution plan is generated to determine the processing mode of each operator in the model. 
OSDP is proposed to make trade-offs between the memory consumption reduction and the hardware efficiency improvement, which maximizes the system throughput. It provides two modes for processing each operator, including Data Parallel (DP) and Zero redundancy Data Parallel (ZDP). As shown in Figure~\ref{fig:DPvsZDP}, they have distinct communication patterns.
During the model initialization and forward processes, both the DP and ZDP operators shard and all-gather their parameters across data parallel process. Full weights of ZDP operators are discarded for memory saving after forward pass. During the backward process, DP operators compute their gradients directly, while ZDP operators all-gather full weights across data parallel process, compute their gradients and then discarded full weights again at the end of backward pass. During gradient synchronization process, both DP and ZDP operators perform reduce-scatter operations across data parallel process to synchronize gradients.

\begin{figure}[t]
\centering
\includegraphics[width=1.0\linewidth]{figure/OSDPworkflow.pdf}
\caption{Workflow of OSDP.}
\vspace{-5mm}
\label{fig:OSDPworkflow}
\end{figure}

Figure~\ref{fig:OSDPworkflow} demonstrates the workflow of OSDP.
It mainly contains three modules: Profiler, Search Engine and Scheduler. The Profiler takes the model description, device information and batch size (initialize as 1) as inputs, and outputs the estimated time and memory cost of each operator with different processing modes as well as the device memory limit. The Search Engine receives the outputs generated from the Profiler, and yields the optimal execution plan and estimated system throughput. The Scheduler takes the outputs of the Search Engine as candidates and iteratively increase the batch size that the Profiler takes as input. As long as the minimum possible memory exceeds the device memory limit, Scheduler selects and outputs the overall optimal execution plan and its corresponding batch size.

We formulate the optimal execution plan searching problem as follows. 
Suppose $O_{i,c,b}$ represents the $i$th operator with mode $c$ under batch size $b$, $t()$ and $m()$ represents the time and memory cost, and $m\_limit$ represents the available device memory. Then we have the following objective:

\vspace{-3mm}
\begin{equation}
    \small
    \begin{split}
    t_{min} &= 
            \mathop{min}\limits_{b\in(0,\infty)}
            \begin{Bmatrix}
            \mathop{min}\limits_{c\in(DP,ZDP)}
            \begin{Bmatrix}
             {\sum_{i=0}^{n-1}{t(O_{i,c,b})}}
            \end{Bmatrix}
            \cdot \frac{1}{b}
            \end{Bmatrix}\\
    & s.t. \qquad {\sum_{i=0}^{n-1}{m(O_{i,c,b})}} \leq m\_limit
    \end{split}
\end{equation}

\begin{figure}
\centering
\includegraphics[width=1.0\linewidth]{figure/OSDP_API.png}
\caption{Comparison between FSDP and OSDP.}
\vspace{-5mm}
\label{fig:OSDP_API}
\end{figure}


The Search Engine adopts Depth Fist Search (DFS) to find the optimal execution plan (details are introduced in the Appendix). The above modules are transparent to the users. We provide users with a concise and convenient API interface to use OSDP for data parallel training. Compared with FSDP, we only need to replace a few lines of code to complete the OSDP deployment. We introduce the API comparison between FSDP and OSDP as shown in \autoref{fig:OSDP_API}.

% \begin{figure}
% \centering
% \includegraphics[width=0.8\textwidth]{figure/DPvsZDP.png}
% \caption{Operator processing in DP and ZDP modes.}
% \label{fig:DPvsZDP}
% \end{figure}


\subsection{Operator Splitting} \label{sec:OP}

Operator splitting aims at further alleviate peak memory footprints during training with only negligible overheads. Existing ZeRO-based systems shard model states across workers during model initialization stage and re-gather them during training stage to maintain a complete model forward and backward.
There is a memory surge during the gathering process.
The gigantic tensors produced by the large operators (e.g., \texttt{MatMul}) could turn into peak memory usage and might exceed the device memory.
For instance, a linear operator of GPT-3 contains 0.6 billion parameters. Therefore, we introduce operator splitting to reduce the impact of gigantic tensors in OSDP.

Operator splitting's core idea is to sequentially process a single \texttt{MatMul} and release memory serially to reduce the peak memory overhead during training. We illustrate the workflow in Figure~\ref{fig:operatorsplittingworkflow}, including three steps: First, both the last dimension of the input data and the first dimension of the operator are partitioned into multiple equal parts according to an artificially determined slice granularity. Then, the computation of each equal part is executed serially. Finally, all computation results are summed as the final output.

% \begin{figure}
% \begin{minipage}[t]{0.49\textwidth}
% \centering
% \includegraphics[width=1\textwidth]{figure/OSAworkflow.png}
% \caption{Operator splitting workflow.}
% \label{fig:osaworkflow}
% \end{minipage}
% \begin{minipage}[t]{0.49\textwidth}
% \centering
% \includegraphics[width=1\textwidth]{figure/OP_workflow.png}
% \caption{Operator processing runtime without vs. with operator splitting.}
% \label{fig:osa_1}
% \end{minipage}
% \end{figure}

Combined with ZDP, operator splitting further optimizes memory surge in training from $size(\text{\texttt{MatMul}})$ to $\frac{size(\text{\texttt{MatMul}})}{slice\;granularity}$, which is especially beneficial for large-scale models. In addition, since our distributed training deployment supports overlap of computation and communication \cite{pytorchdistributed}, as long as communication overhead remains a system bottleneck, the additional computational overhead caused by serial computation and summation can be completely covered, thus the impact of operator splitting on the overall training time is almost negligible.

\subsection{Optimal Sharded Data Parallel with Operator Splitting} \label{sec:OSDP+OP}
The performance of OSDP can be further improved with operator splitting. As operator splitting partitions one operator into multiple slices, OSDP can make fine-grained decisions on each slice. For instance, an operator is partitioned into 4 slices, 1 slice is processed in ZDP mode, and the other 3 slices are processed in DP mode. In this case, OSDP can provide a variety of choices for a single operator rather than two, and search for a finer-grained execution plan for the model. Meanwhile, as mentioned in Section~\ref{sec:OP}, operator splitting minimizes memory surge in training, which provides OSDP with the ability to undertake a larger batch size and further optimize the system throughput.

\begin{figure}[t]
\centering
\includegraphics[width=1.0\linewidth]{figure/OSAworkflow.png}
\caption{Workflow of operator splitting.}
\vspace{-5mm}
\label{fig:operatorsplittingworkflow}
\end{figure}


==> plot/asdps_throughput.tex <==
% \begin{figure}
% \centering
% \begin{minipage}[t]{1\textwidth}
% \centering
% \begin{tikzpicture}
% \centering
% \begin{groupplot}[
%     group style={group size=5 by 1},
%     y axis line style={opacity=0},
%     grid style=dashed,
%     ]
% \nextgroupplot[
%     height=0.25\linewidth,
%     width=0.3\linewidth,
%     ybar,
%     symbolic x coords={0, $[$24 1024$]$, $[$24 1536$]$, max},
%     ymin = 0,
%     xticklabels={},
%     extra x ticks={$[$24 1024$]$, $[$24 1536$]$},
%     extra x tick labels={$[$24 1024$]$, $[$24 1536$]$},
%     xmin = 0,
%     xmax = max,
%     xlabel = {5GB},
%     % label style={font=\tiny},
%     ylabel = {Throughput (seq/s)},
%     ylabel near ticks,
%     bar width=5pt,
%     ymajorgrids,
%     xticklabel style={rotate=45, anchor=east},
%     xlabel style={at={(0.5,-0.5)}},
%     legend style={at={(0.9,1.35)},anchor=north, nodes={scale=0.75, transform shape}},
% ]
% \addplot+[ybar, black] coordinates{($[$24 1024$]$,341.4483623)($[$24 1536$]$,48.48333314)};
% \addplot+[ybar, red] coordinates{($[$24 1024$]$,279.6409885)($[$24 1536$]$,38.42634545)};
% \nextgroupplot[
%     height=0.25\linewidth,
%     width=0.4\linewidth,
%     ybar,
%     symbolic x coords={0, $[$24 1536$]$, $[$24 2048$]$, $[$48 1024$]$, $[$48 1536$]$, max},
%     ymin = 0,
%     xticklabels={},
%     extra x ticks={$[$24 1536$]$, $[$24 2048$]$, $[$48 1024$]$, $[$48 1536$]$},
%     extra x tick labels={$[$24 1536$]$, $[$24 2048$]$, $[$48 1024$]$, $[$48 1536$]$},
%     xmin = 0,
%     xmax = max,
%     xlabel = {10GB},
%     ylabel near ticks,
%     bar width=5pt,
%     ymajorgrids,
%     xticklabel style={rotate=45, anchor=east},
%     xlabel style={at={(0.5,-0.5)}},
%     legend style={at={(0.9,1.35)},anchor=north, nodes={scale=0.75, transform shape}},
% ]
% \addplot+[ybar, black] coordinates{
%     ($[$24 1536$]$,137.7957499)
%     ($[$24 2048$]$,28.19582947)
%     ($[$48 1024$]$,170.7241811)
%     ($[$48 1536$]$,24.24166657)
%     };
% \addplot+[ybar, red] coordinates{
%     ($[$24 1536$]$,124.2848838)
%     ($[$24 2048$]$,21.61481932)
%     ($[$48 1024$]$,139.8204943)
%     ($[$48 1536$]$,19.21317273)
%     };
% \nextgroupplot[
%     height=0.25\linewidth,
%     width=0.35\linewidth,
%     ybar,
%     symbolic x coords={0, $[$24 2048$]$, $[$48 1536$]$, $[$96 1024$]$, max},
%     ymin = 0,
%     xticklabels={},
%     extra x ticks={$[$24 2048$]$, $[$48 1536$]$, $[$96 1024$]$},
%     extra x tick labels={$[$24 2048$]$, $[$48 1536$]$, $[$96 1024$]$},
%     xmin = 0,
%     xmax = max,
%     xlabel = {15GB},
%     ylabel near ticks,
%     bar width=5pt,
%     ymajorgrids,
%     xticklabel style={rotate=45, anchor=east},
%     xlabel style={at={(0.5,-0.5)}},
%     legend style={at={(0.9,1.35)},anchor=north, nodes={scale=0.75, transform shape}},
% ]
% \addplot+[ybar, black] coordinates{
%     ($[$24 2048$]$,67.60632493)
%     ($[$48 1536$]$,44.72839233)
%     ($[$96 1024$]$,67.63213134)
%     };
% \addplot+[ybar, red] coordinates{
%     ($[$24 2048$]$,56.00602625)
%     ($[$48 1536$]$,35.61602465)
%     ($[$96 1024$]$,56.00602625)
%     };
% \legend{ASDPS, FSDP}
% \end{groupplot}
% \end{tikzpicture}
% \end{minipage}
% \begin{minipage}[t]{1\textwidth}
% \centering
% \begin{tikzpicture}
% \centering
% \begin{groupplot}[
%     group style={group size=5 by 1},
%     y axis line style={opacity=0},
%     grid style=dashed,
%     ]
% \nextgroupplot[
%     height=0.25\linewidth,
%     width=0.4\linewidth,
%     ybar,
%     symbolic x coords={0, $[$48 1536$]$, $[$48 2048$]$, $[$96 1536$]$, $[$12 6144$]$, $[$8 8192$]$, max},
%     ymin = 0,
%     xticklabels={},
%     extra x ticks={$[$48 1536$]$, $[$48 2048$]$, $[$96 1536$]$, $[$12 6144$]$, $[$8 8192$]$},
%     extra x tick labels={$[$48 1536$]$, $[$48 2048$]$, $[$96 1536$]$, $[$12 6144$]$, $[$8 8192$]$},
%     xmin = 0,
%     xmax = max,
%     xlabel = {20GB},
%     ylabel near ticks,
%     bar width=5pt,
%     ymajorgrids,
%     xticklabel style={rotate=45, anchor=east},
%     xlabel style={at={(0.5,-0.5)}},
%     legend style={at={(0.9,1.35)},anchor=north, nodes={scale=0.75, transform shape}},
%     ylabel = {Throughput (seq/s)},
% ]
% \addplot+[ybar, black] coordinates{
%     ($[$48 1536$]$,68.89787494)
%     ($[$48 2048$]$,14.10403648)
%     ($[$96 1536$]$,12.12083329)
%     ($[$12 6144$]$, 85.16129032)
%     ($[$8 8192$]$, 68.61255498)
%     };
% \addplot+[ybar, red] coordinates{
%     ($[$48 1536$]$,62.1424419)
%     ($[$48 2048$]$,10.80740966)
%     ($[$96 1536$]$,9.606586363)
%     ($[$12 6144$]$, 61.47232671)
%     ($[$8 8192$]$, 51.92918747)
%     };
% \nextgroupplot[
%     height=0.25\linewidth,
%     width=0.25\linewidth,
%     ybar,
%     symbolic x coords={0, $[$4 12288$]$, max},
%     ymin = 0,
%     xticklabels={},
%     extra x ticks={$[$4 12288$]$},
%     extra x tick labels={$[$4 12288$]$},
%     xmin = 0,
%     xmax = max,
%     xlabel = {24GB},
%     ylabel near ticks,
%     bar width=5pt,
%     ymajorgrids,
%     % xticklabel style={rotate=45, anchor=east},
%     xlabel style={at={(0.5,-0.5)}},
%     legend style={at={(0.9,1.35)},anchor=north, nodes={scale=0.75, transform shape}},
% ]
% \addplot+[ybar, black] coordinates{
%     ($[$4 12288$]$,65.43)
% };
% \addplot+[ybar, red] coordinates{
%     ($[$4 12288$]$,22.3)
% };
% \end{groupplot}
% \end{tikzpicture}
% \end{minipage}
% \caption{Comparison of FSDP and ASDPS throughput under different settings, the x-axis represents different settings for the number of model layers and hidden sizes, the y-axis represents the overall training throughput, and the x labels represent different memory limits.}
% \label{fig:ASDPS_1}
% \end{figure}


\begin{figure*}
\begin{minipage}[t]{1\textwidth}
\centering
\begin{tikzpicture}
\begin{groupplot}[
    group style={group size=5 by 1},
    y axis line style={opacity=0},
    grid style=dashed,
    separate axis lines,
    ]
\nextgroupplot[
    height=0.2\linewidth,
    width=0.3\linewidth,
    ybar,
    symbolic x coords={0, $[$96 1024$]$, mid, $[$48 1536$]$, max},
    % ymin = 0,
    xticklabels={},
    ylabel = {Throughput (seq/s)},
    extra x ticks={$[$96 1024$]$, $[$48 1536$]$},
    extra x tick labels={$[$96 1024$]$, $[$48 1536$]$},
    xmin = 0,
    xmax = max,
    xlabel = {N\&D},
    xlabel near ticks,
    % label style={font=\tiny},
    ylabel near ticks,
    bar width=8pt,
    ymajorgrids,
    % xticklabel style={rotate=30, anchor=east},
    xlabel style={at={(0.5, 1.3)}},
]
\addplot+[ybar, black] coordinates{
    ($[$96 1024$]$,180.8209788)
    ($[$48 1536$]$,170.740416)
};
\addplot+[ybar, red] coordinates{
    ($[$96 1024$]$,214.9018499)
    ($[$48 1536$]$,199.9185413)
};
\addplot+[ybar, pattern={north west lines}, pattern color=red] coordinates{
    ($[$96 1024$]$,221.9575314)
    ($[$48 1536$]$,207.096649)
};
\nextgroupplot[
    height=0.2\linewidth,
    width=0.3\linewidth,
    ybar,
    symbolic x coords={0, $[$4 6144$]$, mid, $[$2 8192$]$, max},
    % ymin = 0,
    xticklabels={},
    extra x ticks={$[$4 6144$]$, $[$2 8192$]$},
    extra x tick labels={$[$4 6144$]$, $[$2 8192$]$},
    xmin = 0,
    xmax = max,
    % label style={font=\tiny},
    ylabel near ticks,
    ymajorgrids,
    % xticklabel style={rotate=30, anchor=east, font=\tiny},
    % xticklabel style={rotate=30, anchor=east},
    bar width=8pt,
    legend entries={FSDP, OSDP, OSDP+OP},
    xlabel = {W\&S},
    % xlabel style={at={(0.5,-0.5)}},
    xlabel near ticks,
    xlabel style={at={(0.5, 1.3)}},
    legend style={at={(0.5,1.6)},anchor=north, nodes={scale=0.75, transform shape}},
    legend columns=-1,
]
\addplot+[ybar, black] coordinates{
    ($[$4 6144$]$,350.5187762)
    ($[$2 8192$]$,392.1754552)
};
\addplot+[ybar, red] coordinates{
    ($[$4 6144$]$,350.5187762)
    ($[$2 8192$]$,392.1754552)
};
\addplot+[ybar, pattern={north west lines}, pattern color=red] coordinates{
    ($[$4 6144$]$,415.5614346)
    ($[$2 8192$]$,670.6373767)
};
\nextgroupplot[
    height=0.2\linewidth,
    width=0.3\linewidth,
    ybar,
    symbolic x coords={0, $[$24 var$]$, mid, $[$48 var$]$, max},
    % ymin = 0,
    xticklabels={},
    extra x ticks={$[$24 var$]$, $[$48 var$]$},
    extra x tick labels={$[$24 var$]$, $[$48 var$]$},
    xmin = 0,
    xmax = max,
    bar width=8pt,
    % label style={font=\tiny},
    ylabel near ticks,
    ymajorgrids,
    xlabel = {I\&C},
    xlabel near ticks,
    xlabel style={at={(0.5, 1.3)}},
    % xticklabel style={rotate=30, anchor=east},
    % xlabel style={at={(0.5, -0.5)}},
    legend style={at={(1.1,1.35)},anchor=north, nodes={scale=0.75, transform shape}},
]
\addplot+[ybar, black] coordinates{
    ($[$24 var$]$,115.7135125)
    ($[$48 var$]$,120.7518505)
};
\addplot+[ybar, red] coordinates{
    ($[$24 var$]$,127.3619366)
    ($[$48 var$]$,128.2660632)
};
\addplot+[ybar, pattern={north west lines}, pattern color=red] coordinates{
    ($[$24 var$]$,141.2889775)
    ($[$48 var$]$,160.0475847)
};
\end{groupplot}
\end{tikzpicture}
\subcaption{Device memory limit 8 GB.}
\end{minipage}
\begin{minipage}[t]{1\textwidth}
\centering
\begin{tikzpicture}
\begin{groupplot}[
    group style={group size=5 by 1},
    y axis line style={opacity=0},
    grid style=dashed,
    separate axis lines,
    ]
\nextgroupplot[
    height=0.2\linewidth,
    width=0.3\linewidth,
    ybar,
    symbolic x coords={0, $[$48 1536$]$, mid, $[$96 1536$]$, max},
    % ymin = 0,
    xticklabels={},
    extra x ticks={$[$48 1536$]$, $[$96 1536$]$},
    extra x tick labels={$[$48 1536$]$, $[$96 1536$]$},
    xmin = 0,
    xmax = max,
    xlabel near ticks,
    ylabel = {Throughput (seq/s)},
    xlabel = {N\&D},
    % xlabel style={font=\tiny},
    ylabel near ticks,
    bar width=8pt,
    ymajorgrids,
    xlabel style={at={(0.5, 1.3)}},
    % xticklabel style={rotate=30, anchor=east},
    % xticklabel style={font=\tiny},
    % xlabel style={at={(0.5,-0.4)}},
    legend style={at={(0.9,1.35)},anchor=north, nodes={scale=0.75, transform shape}},
]
\addplot+[ybar, black] coordinates{
    ($[$48 1536$]$,594.3389498)
    ($[$96 1536$]$,85.37020799)
};
\addplot+[ybar, red] coordinates{
    ($[$48 1536$]$,689.24578)
    ($[$96 1536$]$,99.95927065)
};
\addplot+[ybar, pattern={north west lines}, pattern color=red] coordinates{
    ($[$48 1536$]$,725.70213)
    ($[$96 1536$]$,103.5673309)
};
\nextgroupplot[
    height=0.2\linewidth,
    width=0.3\linewidth,
    ybar,
    symbolic x coords={0, $[$4 8192$]$, mid, $[$2 12288$]$, max},
    % ymin = 0,
    xticklabels={},
    extra x ticks={$[$4 8192$]$, $[$2 12288$]$},
    extra x tick labels={$[$4 8192$]$, $[$2 12288$]$},
    xmin = 0,
    xmax = max,
    xlabel near ticks,
    xlabel = {W\&S},
    % xlabel = {16GB},
    % label style={font=\tiny},
    ylabel near ticks,
    bar width=8pt,
    xlabel style={at={(0.5, 1.3)}},
    ymajorgrids,
    % xticklabel style={rotate=30, anchor=east},
    % xlabel style={at={(0.5,-0.5)}},
    legend style={at={(0.9,1.35)},anchor=north, nodes={scale=0.75, transform shape}},
]
\addplot+[ybar, black] coordinates{
    ($[$4 8192$]$,306.4468119)
    ($[$2 12288$]$,64.4958702)
};
\addplot+[ybar, red] coordinates{
    ($[$4 8192$]$,306.4468119)
    ($[$2 12288$]$,64.4958702)
};
\addplot+[ybar, pattern={north west lines}, pattern color=red] coordinates{
    ($[$4 8192$]$,363.7781997)
    ($[$2 12288$]$,124.0809731)
};
\nextgroupplot[
    height=0.2\linewidth,
    width=0.3\linewidth,
    ybar,
    symbolic x coords={0, $[$48 var$]$, mid, $[$96 var$]$, max},
    % ymin = 0,
    xticklabels={},
    extra x ticks={$[$48 var$]$, $[$96 var$]$},
    extra x tick labels={$[$48 var$]$, $[$96 var$]$},
    xmin = 0,
    xmax = max,
    xlabel near ticks,
    % label style={font=\tiny},
    ylabel near ticks,
    bar width=8pt,
    xlabel = {I\&C},
    xlabel style={at={(0.5, 1.3)}},
    ymajorgrids,
    % xticklabel style={rotate=30, anchor=east},
    % xlabel style={at={(0.5,-0.5)}},
    legend style={at={(0.9,1.35)},anchor=north, nodes={scale=0.75, transform shape}},
]
\addplot+[ybar, black] coordinates{
    ($[$48 var$]$,133.54205123)
    ($[$96 var$]$,79.41265397)
};
\addplot+[ybar, red] coordinates{
    ($[$48 var$]$,145.1447077)
    ($[$96 var$]$,92.12912665)
};
\addplot+[ybar, pattern={north west lines}, pattern color=red] coordinates{
    ($[$48 var$]$,159.402836)
    ($[$96 var$]$,96.05631487)
};
\end{groupplot}
\end{tikzpicture}
\subcaption{Device memory limit 16 GB.}
\end{minipage}
\caption{Comparison of FSDP and OSDP throughput under different settings, the x-axis represents different settings for the number of model layers and hidden sizes, the x label represents the model type, and the y-axis represents the overall training throughput.}
\label{fig:ASDPS_1}
\end{figure*}

==> plot/cpsa_time_and_mem.tex <==
\begin{figure*}
\begin{minipage}[t]{0.24\textwidth}
\centering
\begin{tikzpicture}
    \begin{axis}[
        xlabel={Different decisions},
        ylabel={Time cost (s)}, 
        legend style={at={(0.8,1.35)},anchor=north, nodes={scale=0.5, transform shape}},
        symbolic x coords={0, 1, 2, 3, 4},
        %xtick distance=1.2,
        xticklabels={},
        extra x ticks={0, 1, 2, 3, 4},
        extra x tick labels={0, 1, 2, 3, 4},
        ytick distance=0.01,
        separate axis lines,
        ybar,
        ymajorgrids,
        scale only axis,
        width=0.65\linewidth,
        height=60pt,
        bar width=3pt,
        ymin=0,
        ymax=0.05,
        %ylabel shift=-3pt,
        ylabel near ticks,
        xlabel near ticks,
        %xlabel shift=-5.9pt,
        % xticklabel style={rotate=45, anchor=east},
        %xlabel style={at={(0.5,-0.150)}},
        xtick pos=bottom,
        y axis line style={opacity=0},
        grid style=dashed,
    ]
    \addplot+[ybar, black] coordinates {
        (0, 0.014867014) 
        (1, 0.016773153)
        (2, 0.018905402)
        (3, 0.02100521)
        (4, 0.023751168)
    };
    \addplot+[ybar, red] coordinates {
        (0, 0.029734029) 
        (1, 0.033452963)
        (2, 0.037936065)
        (3, 0.04193049)
        (4, 0.047330852)
    };
    \legend{attn op, mlp op}  
    \end{axis}
\end{tikzpicture}
\subcaption{Impact of different decisions on time.}
\end{minipage}
\begin{minipage}[t]{0.24\textwidth}
\centering
\begin{tikzpicture}
    \begin{axis}[
        xlabel={Different decisions},
        ylabel={Mem cost (MB)}, 
        separate axis lines,
        legend style={at={(0.8,1.35)},anchor=north, nodes={scale=0.5, transform shape}},
        symbolic x coords={0, 1, 2, 3, 4},
        %xtick distance=1.2,
        xticklabels={},
        extra x ticks={0, 1, 2, 3, 4},
        extra x tick labels={0, 1, 2, 3, 4},
        ytick distance=50,
        ybar,
        ymajorgrids,
        scale only axis,
        width=0.65\linewidth,
        height=60pt,
        bar width=3pt,
        ymin=0,
        ymax=260,
        %ylabel near ticks,
        %ylabel shift=-3pt,
        %xlabel shift=-5.9pt,
        % xticklabel style={rotate=45, anchor=east},
        ylabel near ticks,
        xlabel near ticks,
        %xlabel style={at={(0.5,-0.150)}},
        xtick pos=bottom,
        y axis line style={opacity=0},
        grid style=dashed,
    ]
    \addplot+[ybar, black] coordinates {
        (0, 127.0019444) 
        (1, 101.4069444)
        (2, 74.63777778)
        (3, 47.84861111)
        (4, 20.90027778)
    };
    \addplot+[ybar, red] coordinates {
        (0, 251.2730556) 
        (1, 198.2597222)
        (2, 145.7272222)
        (3, 93.37888889)
        (4, 41.80055556)
    };
    \legend{attn op, mlp op} 
    \end{axis}
\end{tikzpicture}
\subcaption{Impact of different decisions on memory.}
\end{minipage}
\begin{minipage}[t]{0.24\textwidth}
\centering
\begin{tikzpicture}
    \begin{axis}[
        xlabel={Different decisions},
        ylabel={Time cost (s)}, 
        separate axis lines,
        legend style={at={(0.8,1.35)},anchor=north, nodes={scale=0.5, transform shape}},
        symbolic x coords={0, 1, 2, 3, 4},
        %xtick distance=1.2,
        xticklabels={},
        extra x ticks={0, 1, 2, 3, 4},
        extra x tick labels={0, 1, 2, 3, 4},
        ytick distance=0.005,
        ybar,
        ymajorgrids,
        scale only axis,
        width=0.65\linewidth,
        height=60pt,
        bar width=3pt,
        ymin=0,
        ymax=0.025,
        %ylabel shift=-3pt,
        ylabel near ticks,
        xlabel near ticks,
        %xlabel shift=-5.9pt,
        % xticklabel style={rotate=45, anchor=east},
        %xlabel style={at={(0.5,-0.150)}},
        xtick pos=bottom,
        y axis line style={opacity=0},
        grid style=dashed,
    ]
    \addplot+[ybar, black] coordinates {
        (0, 0.014867014) 
        (1, 0.016773153)
        (2, 0.018905402)
        (3, 0.02100521)
        (4, 0.023751168)
    };
    \addplot+[ybar, red] coordinates {
        (0, 0.015277778) 
        (1, 0.017152778)
        (2, 0.019027778)
        (3, 0.020902778)
        (4, 0.022777778)
    };
    \legend{actual, predict}  
    \end{axis}
\end{tikzpicture}
\subcaption{Actual vs predict time of attention operator.}
\end{minipage}
\begin{minipage}[t]{0.24\textwidth}
\centering
\begin{tikzpicture}
    \begin{axis}[
        xlabel={Different decisions},
        ylabel={Time cost (s)}, 
        separate axis lines,
        legend style={at={(0.8,1.35)},anchor=north, nodes={scale=0.5, transform shape}},
        symbolic x coords={0, 1, 2, 3, 4},
        %xtick distance=1.2,
        xticklabels={},
        extra x ticks={0, 1, 2, 3, 4},
        extra x tick labels={0, 1, 2, 3, 4},
        ytick distance=0.01,
        ybar,
        ymajorgrids,
        scale only axis,
        width=0.65\linewidth,
        height=60pt,
        bar width=3pt,
        ymin=0,
        ymax=0.05,
        %ylabel shift=-3pt,
        ylabel near ticks,
        xlabel near ticks,
        %xlabel shift=-5.9pt,
        % xticklabel style={rotate=45, anchor=east},
        %xlabel style={at={(0.5,-0.150)}},
        xtick pos=bottom,
        y axis line style={opacity=0},
        grid style=dashed,
    ]
    \addplot+[ybar, black] coordinates {
        (0, 0.029734029) 
        (1, 0.033452963)
        (2, 0.037936065)
        (3, 0.04193049)
        (4, 0.047330852)
    };
    \addplot+[ybar, red] coordinates {
        (0, 0.030555556) 
        (1, 0.034305556)
        (2, 0.038055556)
        (3, 0.041805556)
        (4, 0.045555556)
    };
    \legend{actual, predict}  
    \end{axis}
\end{tikzpicture}
\subcaption{Actual vs predict time of mlp operator.}
\end{minipage}
% \begin{minipage}[t]{0.4\textwidth}
% \centering
% \begin{tikzpicture}
%     \begin{axis}[
%         xlabel={Different decisions},
%         ylabel={Time cost (s)}, 
%         legend columns=-1,
%         legend pos={north west},
%         symbolic x coords={0 0, 1 0, 2 0, 3 0, 4 0, 4 1, 4 2, 4 3, 4 4},
%         %xtick distance=1.2,
%         xticklabels={},
%         extra x ticks={0 0, 1 0, 2 0, 3 0, 4 0, 4 1, 4 2, 4 3, 4 4},
%         extra x tick labels={0 0, 1 0, 2 0, 3 0, 4 0, 4 1, 4 2, 4 3, 4 4},
%         ytick distance=0.5,
%         ybar,
%         ymajorgrids,
%         scale only axis,
%         width=0.8\linewidth,
%         height=67pt,
%         bar width=6pt,
%         ymin=0,
%         ymax=2,
%         %ylabel near ticks,
%         %ylabel shift=-3pt,
%         %xlabel shift=-5.9pt,
%         xticklabel style={rotate=45, anchor=east},
%         %xlabel style={at={(0.5,-0.150)}},
%         ylabel near ticks,
%         xlabel near ticks,
%         xtick pos=bottom,
%     ]
%     \addplot+[ybar, black] coordinates {
%         (0 0, 1.070425034) 
%         (1 0, 1.116172361)
%         (2 0, 1.167346334)
%         (3 0, 1.217741728)
%         (4 0, 1.283644724)
%         (4 1, 1.372899151)
%         (4 2, 1.480493593)
%         (4 3, 1.576359797)
%         (4 4, 1.705968475)
        
%     };
%     \addplot+[ybar, red] coordinates {
%         (0 0, 1.1) 
%         (1 0, 1.145)
%         (2 0, 1.19)
%         (3 0, 1.235)
%         (4 0, 1.28)
%         (4 1, 1.37)
%         (4 2, 1.46)
%         (4 3, 1.55)
%         (4 4, 1.64)
        
%     };
%     \legend{actual, predict}  
%     \end{axis}
% \end{tikzpicture}
% \end{minipage}
\caption{Impact of different decisions on time and memory cost during training as well as effectiveness of the cost model.}
\label{fig:CSPA_123}
\end{figure*}
